Improving Response Selection in Multi-Turn Dialogue Systems by Incorporating Domain Knowledge

Building systems that can communicate with humans is a core problem in Artificial Intelligence. This work proposes a novel neural network architecture for response selection in an end-to-end multi-turn conversational dialogue setting. The architecture applies context level attention and incorporates additional external knowledge provided by descriptions of domain-specific words. It uses a bi-directional Gated Recurrent Unit (GRU) for encoding context and responses and learns to attend over the context words given the latent response representation and vice versa.In addition, it incorporates external domain specific information using another GRU for encoding the domain keyword descriptions. This allows better representation of domain-specific keywords in responses and hence improves the overall performance. Experimental results show that our model outperforms all other state-of-the-art methods for response selection in multi-turn conversations.

==> attention.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{x}
    \toprule
        gui for shutdown try typing sudo shutdown -h now \\
        pci can you put the output of lspci on __url__ and give me the link please \\
        certainly won n't make a difference i m sure but maybe try sudo shutdown -r now shutdown works just fine graphical and command line \\
        i do n't see a line in xorg conf for hsync and vsync do you get the same you d create it i m looking at gentoo and ubuntu forums a sec \\
        can be many reasons of traceroute __url__ you will not get a complete result \\
        \cmidrule{1}
    \bottomrule
    \end{tabular}
    \caption{\ak{Visualization of attention weight in the contexts.}}
    \label{tab:attention_visualization}
\end{table}
